Decoding Emotional Experience through Physiological Signal Processing

There is an increasing consensus among re- searchers that making a computer emotionally intelligent with the ability to decode human affective states would allow a more meaningful and natural way of human-computer interactions (HCIs). One unobtrusive and non-invasive way of recognizing human affective states entails the exploration of how physiological signals vary under different emotional experiences. In particular, this paper explores the correlation between autonomically-mediated changes in multimodal body signals and discrete emotional states. In order to fully exploit the information in each modality, we have provided an innovative classification approach for three specific physiological signals including Electromyogram (EMG), Blood Volume Pressure (BVP) and Galvanic Skin Response (GSR). These signals are analyzed as inputs to an emotion recognition paradigm based on fusion of a series of weak learners. Our proposed classification approach showed 88.1% recognition accuracy, which outperformed the conventional Support Vector Machine (SVM) classifier with 17% accuracy improvement. Furthermore, in order to avoid information redundancy and the resultant over-fitting, a feature reduction method is proposed based on a correlation analysis to optimize the number of features required for training and validating each weak learner. Results showed that despite the feature space dimensionality reduction from 27 to 18 features, our methodology preserved the recognition accuracy of about 85.0%. This reduction in complexity will get us one step closer towards embedding this human emotion encoder in the wireless and wearable HCI platforms.

==> WH'16/figs.tex <==
\newcommand{\figsignals}{
\begin{figure}
  \centering
  \includegraphics[width=\linewidth,trim=0in 0in 0in 0in,
  clip=true]{figures/signals.png}
  \caption{From top to bottom, examples of the three physiological signals under study obtained from dataset II in \cite{ref1}: \textit{electromyogram} (microvolts), \textit{blood volume pressure} (percent reflectance), \textit{galvanic skin response} (micro Siemens). These signals were measured while the participant experienced the eight emotions proposed for recognition. The segments of data corresponding to each emotion are divided by the magenta dashed lines and its corresponding labels are placed at the top of the graph.}
\label{fig:signals}
\end{figure}
}


\newcommand{\figweakAlg}{
\begin{figure*}
  \centering
  \includegraphics[width=0.96\textwidth,trim=0in 0in 0in 0in,
  clip=true]{figures/weakAlg.png}
  \caption{Emotion classification algorithm based on fusion of weak learners. Twenty-day observations of three physiological signals reported in \cite{ref1} are the input to a pre-processing block constituted of filtering, smoothing and segmentation procedures. These pre-processed signals are divided into training set (19-day observations) and test set (1-day observation). For each of these sets, nine features were computed per emotion per observation day. Three specialized weak learners based on linear discriminant classifiers are build for each physiological signal. As a final step, the weighted predictions provided as the outputs of each weak learner are fused to decode eight discrete emotions.}
\label{fig:weakAlg}
\end{figure*}
}


\newcommand{\figfusionAlg}{
\begin{figure*}
  \centering
  \includegraphics[width=0.96\textwidth,trim=0in 0in 0in 0in,
  clip=true]{figures/fusionAlg.png}
  \caption{Fusion Algorithm -- Given a test input containing the EMG, BVP and GSR signals, each weak learner provides a weighted prediction of the 8 emotions that the input is likely to be constituted of. Next, all the weighted predictions from the 3 weak learners are concatenated in a matrix in order to compute a mean weigh vector that will consolidate these three different criteria. Finally, an discrete 8-emotion classification is obtained by computing the emotion for which the maximum mean weight was computed.}
\label{fig:fusionAlg}
\end{figure*}
}

\newcommand{\figtprFpr}{
\begin{figure}
  \centering
  \includegraphics[width=0.5\textwidth,trim=0in 0in 0in 0in,
  clip=true]{figures/tprFpr.png}
  \caption{
    True Positive Rate -- TPR (solid lines) and False Positive Rate -- FPR (dashed lines) curves for each of the eight target emotions under the scope of the three classifiers under comparison. Note that the proposed weak learners with and without correlation analysis outperform SVM by achieving a higher TPR and lower FPR.}
\label{fig:tprFpr}
\end{figure}
}


\newcommand{\figmisclassification}{
\begin{figure*}
  \centering
  \includegraphics[width=1.0\textwidth,trim=0in 0in 0in 0in,
  clip=true]{figures/misclassificationEmotions.png}
  \caption{Misclassification rates (MSCR) for each of the eight target emotions under analysis when compared with the other seven remaining emotions. For instance, it can be observed that the emotion with the lowest TPR of 0.7, romantic love, is misclassified mainly with anger, joy and in lesser degree by hate and platonic love.}
\label{fig:misclassification}
\end{figure*}
}

\newcommand \figmethod[3]{
\begin{figure*}
  \centering
  \includegraphics[width=0.96\textwidth,  trim=0in 0in 0in 0in,
  clip=true]{figures/#1}
  \caption{#2}
\label{#3}
\end{figure*}
}


==> WH'16/tabs.tex <==
\newcommand{\tblaccuracy}{
\begin{table}[b]
  \centering
  \caption{Comparison between different classifiers' recognition performance} 
  \begin{tabular}{|l|c|}
  \hline
  \textbf{Classifier} & \textbf{Accuracy (\%)}\\
  \hline
  SVM - Linear kernel & 70.0\\
  SVM - Radial basis kernel & 72.5\\
  SVM - 1$^{st}$ order polynomial kernel &68.1\\
  SVM - 2$^{nd}$ order polynomial kernel &70.0\\
  SVM - 3$^{rd}$ order polynomial kernel &71.9\\
  SVM - 4$^{th}$ order polynomial kernel &69.4\\
  SVM - 5$^{th}$ order polynomial kernel &67.5\\
  \hline
  Weak Learners & 88.1\\
  Weak Learners \& Correlation Analysis & 85.0\\
  \hline    
  \end{tabular}
  \label{tbl:accuracy}
\end{table}
}


\newcommand{\tblmisclassification}{
\begin{table}
  \centering
  \caption{The sources of misclassification for the emotions that achieved a TRP lower than 0.9} 
  \begin{tabular}{|l|l|c|}
  \hline
  \textbf{Emotion (TPR)} & \textbf{Misclassification Source} & \textbf{MSCR}\\
  \hline
  Romantic Love (0.70)  & Anger    & 0.10\\
                 & Joy             & 0.10\\
                 & Hate            & 0.05\\
                 & Platonic love   & 0.05\\
  \hline
  Joy (0.75)     & Romantic love     & 0.15\\
                 & Grief             & 0.05\\
                 & Platonic love     & 0.05\\
  \hline
  Hate (0.75)    & Baseline (N.E.)   & 0.15\\
                 & Reverence         & 0.10\\
  \hline  
  Platonic love (0.85)  & Grief      & 0.10\\
                        & Joy        & 0.05\\
  \hline  
  Reverence (0.85)      & Hate              & 0.10\\
                        & Baseline (N.E.)   & 0.05\\
  \hline    
  \end{tabular}
  \label{tbl:misclassification}
\end{table}
}
